PREDILECT: Preferences Delineated with Zero-Shot Language-based Reasoning in Reinforcement Learning

Preference-based reinforcement learning (RL) has emerged as a new field in robot learning, where humans play a pivotal role in shaping robot behavior by expressing preferences on different sequences of state-action pairs. However, formulating realistic policies for robots demands responses from humans to an extensive array of queries. In this work, we approach the sample-efficiency challenge by expanding the information collected per query to contain both preferences and optional text prompting. To accomplish this, we leverage the zero-shot capabilities of a large language model (LLM) to reason from the text provided by humans. To accommodate the additional query information, we reformulate the reward learning objectives to contain flexible highlights -- state-action pairs that contain relatively high information and are related to the features processed in a zero-shot fashion from a pretrained LLM. In both a simulated scenario and a user study, we reveal the effectiveness of our work by analyzing the feedback and its implications. Additionally, the collective feedback collected serves to train a robot on socially compliant trajectories in a simulated social navigation landscape. We provide video examples of the trained policies at https://sites.google.com/view/rl-predilect

==> content/05simulations.tex <==

\section{Simulated Experiments} \label{sec:simexp}
To determine the efficiency of our method we run simulated experiments to validate the following hypotheses:
\begin{itemize}
    \item \textbf{H1}: POLITE has better sample efficiency than baseline preference learning, by prompting humans fewer times while gathering additional information per preference given. 
    \item \textbf{H2}: POLITE significantly outperforms baseline preference learning by converging faster under the same settings.
\end{itemize}

\subsection{Setup} \label{sec:simexp-setup}


\begin{itemize}
  \item PREDILECT (Our method): using highlighted queries as described in section \ref{sec:polite}.
  \item Preference Learning (Baseline): Preference learning based on the work of Christiano et al. \cite{christiano2017deep}, which can be considered an ablation of PREDILECT without highlights and exclusively using Eq.\ref{eq:preferenceloss} for the learning objective of $\rewardnetwork$.
\end{itemize}

\subsection{Result}




\label{sec:simulationresult}

